Assessing the robustness of parsimonious predictions for gene neighborhoods from reconciled phylogenies

The availability of a large number of assembled genomes opens the way to study the evolution of syntenic character within a phylogenetic context. The DeCo algorithm, recently introduced by B{\'e}rard et al. allows the computation of parsimonious evolutionary scenarios for gene adjacencies, from pairs of reconciled gene trees. Following the approach pioneered by Sturmfels and Pachter, we describe how to modify the DeCo dynamic programming algorithm to identify classes of cost schemes that generates similar parsimonious evolutionary scenarios for gene adjacencies, as well as the robustness to changes to the cost scheme of evolutionary events of the presence or absence of specific ancestral gene adjacencies. We apply our method to six thousands mammalian gene families, and show that computing the robustness to changes to cost schemes provides new and interesting insights on the evolution of gene adjacencies and the DeCo model.

==> conclusion_isbra.tex <==
% !TeX root = DeClope.tex 

In the present work, we consider the robustness of the predictions of the
\DeCo{}~\citep{DBLP:journals/bioinformatics/BerardGBSDT12} to perturbations of 
the evolutionary cost model algorithm.  To that purpose, we adapt an
algebraic geometry framework for dynamic programming, pioneered
by~\cite{PachterS2005}, and use it to fully partition the space of
cost schemes.  We define objective, efficiently computed, measures of
robustness for features (ancestral adjacency, event counts) of
evolutionary scenario.  Together with the ensemble approach described
in~\citep{DBLP:conf/wob/ChauvePZ14}, this provides tools that extend
and complement the parsimonious approach to study the evolution of
syntenic
characters~\citep{DBLP:journals/bioinformatics/BerardGBSDT12}. Our
analysis of a set of mammalian reconciled gene trees provides useful
insights on this dataset, especially by revealing that a large
majority of instances are extremely robust to a change in cost scheme,
as are a large number of inferred ancestral adajcencies. 

